Enhancing key rates of QKD protocol by Coincidence Detection

In theory, quantum key distribution (QKD) provides unconditional security; however, its practical implementations are susceptible to exploitable vulnerabilities. This investigation tackles the constraints in practical QKD implementations using weak coherent pulses. We improve on the conventional approach of using decoy pulses by integrating it with the coincidence detection (CD) protocol. Additionally, we introduce an easy-to-implement algorithm to compute asymptotic key rates for the protocol. Furthermore, we have carried out an experimental implementation of the protocol, where we demonstrate that monitoring coincidences in the decoy state protocol leads to enhanced key rates under realistic experimental conditions.

==> Packages.tex <==
\usepackage[numbers,sort&compress]{natbib} 
\usepackage[compact]{titlesec}
\usepackage[utf8]{inputenc}
\usepackage{hyperref}
\usepackage{url}
\usepackage{times}
\usepackage{tikz}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subfigure}
\usepackage{float}
\usepackage{stfloats}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{physics}
\usepackage{braket}
\usepackage{bm}
\usepackage{breqn}
\usepackage{array}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{dcolumn}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{textcomp}
\usepackage{soul}
\usepackage{ulem}
\usepackage{gensymb}
\usepackage{ragged2e}
\usepackage{upgreek}
\usepackage{fancyhdr}
\usepackage{comment}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage{bbold}
\usepackage{verbatim}
\usepackage{balance}
\usepackage{algorithm}
\usepackage{algorithmic}
\newcommand{\bin}{\mathrm{bin}}
